Semi-bandit Optimization in the Dispersed Setting

The goal of data-driven algorithm design is to obtain high-performing algorithms for specific application domains using machine learning and data. Across many fields in AI, science, and engineering, practitioners will often fix a family of parameterized algorithms and then optimize those parameters to obtain good performance on example instances from the application domain. In the online setting, we must choose algorithm parameters for each instance as they arrive, and our goal is to be competitive with the best fixed algorithm in hindsight. There are two major challenges in online data-driven algorithm design. First, it can be computationally expensive to evaluate the loss functions that map algorithm parameters to performance, which often require the learner to run a combinatorial algorithm to measure its performance. Second, the losses can be extremely volatile and have sharp discontinuities. However, we show that in many applications, evaluating the loss function for one algorithm choice can sometimes reveal the loss for a range of similar algorithms, essentially for free. We develop online optimization algorithms capable of using this kind of extra information by working in the semi-bandit feedback setting. Our algorithms achieve regret bounds that are essentially as good as algorithms under full-information feedback and are significantly more computationally efficient. We apply our semi-bandit results to obtain the first provable guarantees for data-driven algorithm design for linkage-based clustering and we improve the best regret bounds for designing greedy knapsack algorithms.

==> definitions.tex <==

In this section we introduce two refined dispersion definitions similar in
spirit to  $(w,k)$-dispersion introduced by \citet{Balcan17:Dispersion}. For
online optimization of piecewise Lipschitz functions it is not possible to
achieve sublinear regret against worst-case adversaries. Recall that a sequence
of functions $\ell_1, \dots, \ell_T$ is $(w,k)$-dispersed if no Euclidean ball
$B(\rho, w)$ of radius $w$ in the parameter space contained discontinuities for
more than $k$ of the functions. Intuitively, when the functions are
$(w,k)$-dispersed for large values of $w$ and $k$, this implies that the
discontinuities of the functions are ``spread out''. \citet{Balcan17:Dispersion}
provide algorithms with sublinear regret bounds under both full-information and
bandit feedback whenever the adversary chooses sequences of functions that are
$(w,k)$-dispersed for suitable values of $w$ and $k$. Our refined definitions
clarify the interdependence of $w$, $k$, and $T$ and cleanly characterize the
necessary dispersion needed for sublinear regret.

Both of our refined definitions capture the expected maximum rate at which we
encounter functions with discontinuities in balls of radius $\epsilon$, as a
function of both time, $T$, and the radius of the ball, $\epsilon$. The first
version, $\beta$-dispersion, cleanly characterizes the the exponent on $T$ in
our regret bounds in terms of the dispersion properties of the sequence of loss
functions. Our second definition, $f$-dispersion, is more general than both
$(w,k)$ and $\beta$-dispersion.

For the remainder of this section, we consider a possibly random sequence of
piecewise Lipschitz loss functions $\ell_1, \ell_2, \dots$ mapping the parameter
space $\configs \subset \reals^d$ to bounded losses in $[0,1]$.

Our first definition is a modification of the dispersion definition introduced
by \citet{Balcan17:Dispersion} that captures the important properties
characterizing the asymptotic regret bounds. We use the notation $\tilde
O(\cdot)$ to suppress all logarithmic terms, and all parameters other than the
time horizon $T$ and the dimension $d$ of the parameter space, which are the
most important terms in our regret bounds.

\begin{definition}\label{def:betadisp}
  %
  The sequence $\ell_1,\ell_2,\dots$ is \emph{$\beta$-dispersed} for the
  Lipschitz constant $L$ if for all $T$ and for all $\epsilon \geq T^{-\beta}$, we
  have that, in expectation, the maximum number of functions among
  $\ell_1,\dots,\ell_T$ which are not $L$-Lipschitz in any $\epsilon$-ball of
  $\configs$ is at most $\tilde O(\epsilon T)$. In other words, we require for
  all $T$ and for all $\epsilon \geq T^{-\beta}$ that
  %
  \[
    \expect \left[
      \max_{\rho\in \configs}(\scount{1\leq i\leq T\mid \ell_i\text{ is not $L$-Lipschitz in }B(\rho,\epsilon)}
    \right]
    =\tilde O(\epsilon T).
  \]
  %
\end{definition}

In all of the online optimization problems we consider, the sequence of loss
functions $\ell_1, \ell_2, \dots$ is random due to smoothness assumptions on the
adversary, and the expectation is over this randomness. This is a stronger
condition for larger $\beta$, since then the inequality holds for smaller balls.
When the loss functions are $\beta$-dispersed, our semi-bandit optimization
algorithm has regret bounded by $\tilde O(\sqrt{Td} + T^{1-\beta})$.

Our next definition is a generalization of both $\beta$ and $(w,k)$-dispersion
that will lead to our sharpest regret bounds in each application.

\begin{definition}\label{fdisp}
  %
  The sequence $\ell_1,\ell_2,\dots$ is \emph{$f$-dispersed} for the Lipschitz
  constant $L$ and dispersion function $f : \mathbb{N} \times [0,\infty) \to
  \reals$ if for all $T$ and for all $\epsilon > 0$, we have that, in
  expectation, the maximum number of functions among $\ell_1,\dots,\ell_T$ which
  are not $L$-Lipschitz in any single $\epsilon$-ball of $\configs$ is at most
  $f(T, \epsilon)$. In other words, we require for all $T$ and for all $\epsilon
  > 0$ that
  %
  \[
    \expect \left[
      \max_{\rho\in \configs}(\scount{1\leq i\leq T\mid \ell_i\text{ is not $L$-Lipschitz in }B(\rho,\epsilon)}
    \right]
    \leq f(T, \epsilon).
  \]
  %
\end{definition}

Note that we may always assume that the function $f$ is a non-decreasing
function of both $T$ and $\epsilon$, since considering longer sequences of
functions or larger balls can only increase the number of non-Lipschitz
functions per ball.

We can express both $(w,k)$-dispersion and $\beta$-dispersion in terms of
$f$-dispersion. In particular, suppose that the functions $\ell_1, \ell_2,
\dots$ are $\beta$-dispersed. Then for any $\epsilon \geq T^{-\beta}$, at most
$\tilde O(\epsilon T)$ of the functions are not Lipschitz on the worst ball of
radius $\epsilon$. In particular, for $\epsilon = T^{-\beta}$, this gives that
the number of non-Lipschitz functions is bounded by $T^{1-\beta}$. For all
radiuses $\epsilon$ smaller than $T^{-\beta}$, this bound also applies, since
decreasing the radius can only decrease the number of non-Lipschitz functions.
It follows that the functions are $f$-dispersed for $f(T,\epsilon) = \tilde
O(\epsilon T + T^{1-\beta})$. Next, suppose $\ell_1, \ell_2, \dots$ are $(w,
k)$-dispersed. Then they are $f$-dispersed for
%
\[
  f(T,\epsilon)
    = \begin{cases} k & \hbox{if $\epsilon \leq w$} \\
    T & \hbox{otherwise,}
  \end{cases}
\]
%
which requires that the maximum number of non-Lipschitz functions in any ball of
radius $\epsilon$ is at most $k$ whenever $\epsilon \leq w$ and otherwise it
allows every function to be non-Lipschitz.


==> discretization.tex <==
In this section we provide a single algorithm that has regret bounds for the
full-information, semi-bandit feedback, and bandit-feedback settings. The high
level idea is to reduce the problem to a finite-armed bandit and apply the
Exp3-SET algorithm of \citet{Alon17:GraphFeedback}, which enjoys regret bounds
in all three of these settings. In particular, we choose a value of $r > 0$ and
construct a $r$-net for the parameter space $\configs$ (which can be done using
at most $(3R/r)^d$ points when $\configs$ is contained in a ball of radius $R$
in $d$ dimensions. Then we run the Exp3-SET algorithm over this finite set).
Exp3-SET is guaranteed to have bounded regret compared to the best point from
the $r$-net, and we use $f$-dispersion to bound the expected difference in total
loss between the best discretized point and the best point in all of $\configs$
by $TLr + f(T,r)$. We then get bounds for each of the three feedback regimes by
tuning the parameters $r$ and $\lambda$ of this single algorithm.

On each round, we assume that the learner observes a feedback set $A_t$,
together with the loss $\ell_t(\rho)$ for all points $\rho \in A_t$. In the full
information setting, we take $A_t = \configs$ to be the entire parameter space.
In the bandit feedback setting, we take $A_t = \{\rho_t\}$, where $\rho_t$ is
the point played by the learner in round $t$. And in the semi-bandit feedback
setting, we take $A_t$ to be the piece of $\ell_t$ that contains the point
$\rho_t$ played by the learner. Using this notation, pseudocode is given in
\Cref{alg:discretizedExp3Set}.

\begin{algorithm}
\noindent \textbf{Parameters:} Granularity $r > 0$, step size $\lambda \in [0,1]$
\begin{enumerate}[nosep, leftmargin=*]
\item Let $\hat \rho_1, \dots \hat \rho_N$ be an $r$-net for $\configs$ of size $N \leq \bigl(\frac{3R}{r}\bigr)^d$.
\item Let $w_{i,1} = 1$ for all $i = 1, \dots, N$.
\item For $t = 1, \dots, T$
  \begin{enumerate}[nosep, leftmargin=*]
  \item Let $p_{i,t} = w_{i,t} / W_t$, where $W_t = \sum_i w_{i,t}$.
  \item Let $\rho_t = \hat \rho_i$ with probability $p_{i,t}$ and play $\rho_t$.
  \item Observe feedback set $A_t$ and $\ell_t(\hat \rho_i)$ for all $\hat \rho_i \in A_t$.
  \item Let $\hat \ell_{i,t} = \frac{\ind{\hat \rho_i \in A_t}}{q_t} \ell_t(\hat \rho_i)$, where $q_t = \sum_{i : \hat \rho_i \in A_t} p_{i,t}$.
  \item Let $w_{i,t+1} = w_{i,t} \exp(-\lambda \hat \ell_{i,t})$ for all $i = 1, \dots, N$.
  \end{enumerate}
\end{enumerate}
\caption{Discretized Exp3-SET}
\label{alg:discretizedExp3Set}
\end{algorithm}

\begin{theorem} \label{thm:discretizedRegret}
  %
  Let $\configs \subset \reals^d$ be contained in a ball of radius $R$ and
  $\ell_1, \dots, \ell_T$ be possibly random piecewise $L$-Lipschitz functions
  that are $f$-dispersed and have an $r_0$-interior optimum. Then running
  \Cref{alg:discretizedExp3Set} with discretization parameter $r \leq r_0$, the
  following claims hold:
  %
  \begin{enumerate}
  %
  \item Under full information, setting $r = 1/(L\sqrt{T})$ and $\lambda =
  \sqrt{\ln(RL\sqrt{T})/T}$ gives expected regret bounded by $O(\sqrt{dT
  \log(RLT)} + f(T, 1/(L\sqrt{T}))$.
  %
  \item Under semi-bandit feedback, if each function $\ell_t$ has at most $M$
  pieces, setting $r = 1/(L \sqrt{T})$ and $\lambda = \sqrt{d \ln(RL\sqrt{T}) /
  (MT)}$ gives expected regret bounded by $O(\sqrt{dTM \log(RLT)} + f(T, 1/(L
  \sqrt{T}))$.
  %
  \item Under bandit feedback, setting $r = T^{\frac{d+1}{d+2}/2} =
  T^{-1/(d+2)}$ and $\lambda = \sqrt{d \ln(3RT^{\frac{1}{d+2}})/((3R)^d
  T^{\frac{2(d+1)}{d+2}})}$ gives expected regret bounded by
  $O\left(T^{\frac{d+1}{d+2}}(d (3R)^d \ln(RT) + L) + f(T,
  \frac{1}{T^{1/(d+2)}})\right)$.
  %
  \end{enumerate}
  %
\end{theorem}

In each of the above bounds, the role of the dispersion parameter $f$ is clean.
For both the full-information and semi-bandit feedback settings, the only term
in the bound that depends on $f$ is the $f(T, 1/(L\sqrt{T}))$ term. Similarly,
for bandit  feedback, the bound depends on $f$ only through the $f(T,
1/T^{1/(d-2)})$ term. In either case, it is clear that the regret bound after
$T$ rounds depends on the dispersion properties in neighborhoods of radius
$1/(L\sqrt{T})$ and $1/T^{1/(d-2)}$, respectively. We know that the function
$f(T,\epsilon)$ should be non-decreasing in the parameter $\epsilon$, so this
also shows that in one sense we require ``less'' dispersion in the bandit
setting, since the bandit bounds depend on $f(T, 1/T^{1/(d+2)}) \leq f(T,
1/\sqrt{T}))$.

\begin{proof}
  %
  Let $\ell_1, \dots, \ell_T$ be the sequence of loss functions. By assumption,
  with probability one there is an optimal parameter in hindsight $\rho^*$ such
  that $B(\rho^*, r) \subset \configs$. It follows that at least one of the
  discretization points $\hat \rho_1, \dots, \hat \rho_N$ must belong to this
  ball. Let $\hat \rho^*$ be such a point. We use $f$-dispersion to argue that
  the total loss of $\hat \rho^*$ is not much more than the total loss of
  $\rho^*$ in expectation over the loss functions $\ell_t$.  Let
  %
  \[
  D = \scount{1 \leq t \leq T \,:\, \ell_t \hbox{ is not $L$-Lipschitz on $B(\rho^*, r)$}}
  \]
  %
  be the number of loss functions that are not $L$-Lipschitz on $B(\rho^*,
  r)$. We know that $\sum_{t=1}^T \ell_t(\hat \rho^*) - \ell_t(\rho^*) \leq TLr
  + D$, since $D$ of the functions have discontinuities and the remaining $T-D <
  T$ are $L$-Lipschitz. Taking the expectation over $\ell_1, \dots, \ell_T$ and
  using the fact that $\expect[D] \leq f(T, r)$, we have that
  %
  \begin{equation}
  \expect\left[\sum_{t=1}^T \ell_t(\hat \rho^*) - \ell_t(\rho^*)\right] \leq TLr + f(T, r).
  \label{eq:discreteOptimality}
  \end{equation}
  %
  Therefore, it is sufficient to show that \Cref{alg:discretizedExp3Set} is
  competitive with $\rho^*$ in expectation over the algorithm randomness.


  \Cref{alg:discretizedExp3Set} runs a special case of the Exp3-SET algorithm of
  \citet{Alon17:GraphFeedback} over the discretized set of parameters $\hat
  \rho_1, \dots, \hat \rho_N$. In particular, we have assumed that the feedback
  system takes a particular form: on each round the arms are partitioned into
  sets such that playing any arm from one set reveals the loss for all arms in
  the same set. \citet{Alon17:GraphFeedback} bound the regret of this algorithm
  for a broader class of feedback systems, where on every round there is an
  undirected graphs defined over the arms fo the bandit and playing an arm
  reveals not only its loss, but also the loss of all adjacent arms in the
  feedback graph $G_t$. Our special case corresponds to the setting where $G_t$
  is the union of several cliques (in the full-information setting, $G_t$ is the
  complete graph, in the semi-bandit setting, $G_t$ is the union of $M$ cliques,
  where $M$ is the number of pieces, and in the bandit setting, $G_t$ is the
  union of $N$ cliques, each consisting of a single node). Corollary 3 of
  \citep{Alon17:GraphFeedback} bound the regret of the algorithm by
  %
  \[
  \expect\left[\sum_{t=1}^T \ell_t(\rho_t)\right] - \sum_{t=1}^T \ell_t(\hat \rho^*)
  \leq \frac{1}{\lambda} \ln(N) + \frac{\lambda}{2} \sum_{t=1}^T \alpha(G_t),
  \]
  %
  where $\alpha(G_t)$ is the size of the largest independent set in the feedback
  graph $G_t$ at round $t$ and the expectation is over the randomness of the
  algorithm, and holds for any oblivious choice of loss functions $\ell_1,
  \dots, \ell_T$ and feedback graphs $G_1, \dots, G_T$. In particular, if
  $\alpha(G_t) \leq \alpha$ for some number $\alpha$ on all time steps, then
  setting $\lambda = \sqrt{\ln(N)/(T\alpha)}$ gives
  %
  \[
  \expect\left[\sum_{t=1}^T \ell_t(\rho_t)\right] - \sum_{t=1}^T \ell_t(\hat \rho^*)
  \leq O(\sqrt{\ln(N) T \alpha}).
  \]
  %
  Finally, taking expectations over the randomness in the loss functions
  $\ell_1, \dots, \ell_T$, using \eqref{eq:discreteOptimality}, the above
  choice of $\lambda$, and the fact that $N \leq (3R/r)^d$, we have
  %
  \[
  \expect\left[\sum_{t=1}^T \ell_t(\rho_t) - \ell_t(\rho^*) \right]
  \leq O\left(\sqrt{d T \alpha \ln(R/r)} + TLr + f(T,r)\right)
  \]

  \vspace{1em}\noindent\textit{Full information.} In the full information
  setting, the feedback graph $G_t$ is the complete graph, for which the largest
  independent set is of size $\alpha = 1$. In this case, choosing $r = 1/(L
  \sqrt{T})$ leads to $\lambda = \sqrt{\ln(RL\sqrt{T})/T}$ and gives
  expected regret bounded by $O(\sqrt{dT \log(RLT)} + f(T,1/(L\sqrt{T}))$.

  \vspace{1em}\noindent\textit{Semi-bandit feedback.} Next suppose that each
  function $\ell_t$ is piecewise defined with at most $M$ and when the learner
  plays a point $\rho_t$, they learn the loss for all points belonging to the
  same piece. In this case, the feedback graph $G_t$ consists of the union of
  $M$ cliques, and the largest independent set has size at most $\alpha = M$.
  Again, choosing $r = 1/(L \sqrt{T})$ leads to $\lambda = \sqrt{d
  \ln(RL\sqrt{T}) / (MT)}$ and gives expected regret bound by $O(\sqrt{d T M
  \log(RLT)} + f(T, 1/(L \sqrt{T}))$.

  \vspace{1em}\noindent\textit{Bandit feedback.} Finally, consider the bandit
  feedback setting. In this case, the feedback graph $G_t$ has the empty
  edge-set and therefore the largest independent set is of size $\alpha = N \leq
  (3R/r)^d$ (the total number of arms). Choosing $r = T^{\frac{d-1}{d-2}-1}$
  leads to
  %
  \[
    \lambda = \sqrt{\frac{d \ln(3RT^{\frac{1}{d+2}})}{(3R)^d T^{\frac{2(d+1)}{d+2}}}}
  \]
  %
  and expected regret bounded by $O\left(T^{\frac{d+1}{d+2}}(d (3R)^d \ln(RT) +
  L) + f(T, \frac{1}{T^{1/(d+2)}})\right)$.
  %
\end{proof}

Note, the condition that $B(\rho^*, r_0) \subset \configs$ with probability one
is only for technical convenience. We can always modify the optimization problem
so that this condition is satisfied. In particular, we define an enlarged
parameter space $\configs' = \bigcup_{\rho \in \configs} B(\rho, r_0)$ and
replace the utility function $u_t$ with its Lipschitz extension to $\configs'$.
On this modified problem we are guaranteed that there exists an optimal
parameter in the $r_0$-interior of $\configs'$, and the Lipschitz-extended
functions are still piecewise Lipschitz and $f$-dispersed for the same $f$.


==> oneDimensionalImplementation.tex <==
In this section we show how to use the modified interval tree data structure of
\citet{Cohen-Addad17:Online} to implement the continuous Exp3-SET algorithm
efficiently for one-dimensional problems with piecewise constant loss functions.
In particular, the per-round cost of updating the algorithm weights and sampling
from them at time $t$ is only $O(\log(t))$, while a direct implementation has
running time given by $O(t)$ instead. We also show how to use interval trees to
implement the Exp3 algorithm on a set of $N$ arms with per-round running time
that is $O(\log N)$, which implies that a discretization-based algorithm in the
bandit setting can be efficiently implemented even in high dimensions.

\paragraph{Interval Tree Summary.} \citet{Cohen-Addad17:Online} introduce a modified
interval tree data structure used for representing piecewise constant functions
mapping $\reals$ to $\reals$. Their data structure represents the function as a
balanced tree with one leaf corresponding to each constant interval of the
function. It supports two main operations called \textsc{Draw} and
\textsc{Update}:
%
\begin{itemize}
%
\item The \textsc{Draw} procedure returns a sample from the density function
that is proportional to the represented piecewise constant function $f$.
%
\item The \textsc{Update} procedure takes an interval $[a,b)$ and an update $u$,
and updates the represented piecewise function by multiplying the function
values in $[a,b)$ by $u$. That is, if the represented function was originally
$f : \reals \to \reals$, after executing \textsc{Update} with interval $[a,b)$
and update $u$, the resulting function is
%
\[
  f'(x) = \begin{cases}
    f(x) & \text{if $x \not \in [a,b)$} \\
    u\cdot f(x) & \text{if $x \in [a,b)$}.
  \end{cases}
\]
%
\end{itemize}
%
\citet{Cohen-Addad17:Online} show that the operations \textsc{Draw} and
\textsc{Update} can be implemented in $O(\log P)$ time, where $P$ is the number
of constant pieces in the represented function. The data structure also makes it
possible to implement a third procedure \textsc{Integrate} in $O(\log P)$ time,
which takes an interval $[a,b)$ and returns the integral of the represented
represented function on the interval $[a,b)$.

\paragraph{Exp3-Set for Piecewise Constant One Dimensional Problems.} First, we
show how to efficiently implement \Cref{alg:cExp3Set} efficiently for
one-dimensional optimization problems with piecewise constant loss functions. We
simply use the interval tree datastructure of \citet{Cohen-Addad17:Online} to
represent the weight function at each round. Pseudocode is given in
\Cref{alg:IntervalExp3Set}.

\begin{lemma}
  %
  Consider an online optimization problem with loss functions $\ell_1, \ell_2 :
  [0,1] \to [0,1]$ that are piecewise constant. Moreover, suppose that on each
  round $t$, the loss $\ell_t$ is constant on each of the feedback sets
  $A^{(t)}_i$. For such a problem, \Cref{alg:IntervalExp3Set} is equivalent to
  \Cref{alg:cExp3Set}. The overhead of sampling and updating the weights on
  round $t$ takes $O(\log t)$ time.
  %
\end{lemma}
\begin{proof}
  %
  On each round we run $\textsc{Update}$ once to update the interval tree. This
  at most increases the number of constant intervals in the weights by 2, since
  the only constant intervals that might get split are the two containing the
  end points of the feedback set $A_t$. Therefore, on round $t$, the weight
  function is piecewise constant with at most $O(2t)$ intervals. It follows that
  the sampling, integration, and update operations all take $O(\log t)$ time,
  giving a total per-round cost of $O(\log t)$.
  %
\end{proof}

\begin{algorithm}
\noindent \textbf{Parameter:} Step size $\lambda \in [0,1]$
\begin{enumerate}[nosep, leftmargin=*]
\item Initialize $W$ to be the interval tree representing $w(\rho) = \ind{\rho \in [0,1]}$.
\item For $t = 1, \dots, T$
  \begin{enumerate}[nosep, leftmargin=*]
  \item Let $\rho_t \leftarrow \textsc{Draw}(W)$ and play $\rho_t$.
  \item Observe feedback interval $A_t = A^{(t)}(\rho)$ and loss $\ell_t(\rho_t)$.
  \item Let $\hat \ell_t \leftarrow \frac{\ell_t(\rho_t)}{p_t(A_t)}$, where $p_t(A_t) \leftarrow \frac{\textsc{Integrate}(W, A_t)}{\textsc{Integrate}(W, [0,1])}$.
  \item Call $\textsc{Update}(W, A_t, \hat \ell_t)$.
  \end{enumerate}
\end{enumerate}
\caption{Continuous Exp3-SET for Piecwise Constant One Dimensional Problems}
\label{alg:IntervalExp3Set}
\end{algorithm}

\paragraph{Efficient Implementation of Exp3.} Next, we show how to implement the
finite-armed Exp3 algorithm using interval trees with per-round running time
that is logarithmic in the number of arms, $N$. The idea is to associate arm $i$
of the bandit with the interval $[(i-1)/N, i/N) \subset [0,1]$ and use the
modified interval tree data structure to efficiently store the weights of the
arms and to do the sampling. Pseudocode for this implementation is given in
\Cref{alg:IntervalExp3}.

\begin{lemma}
  %
  \Cref{alg:IntervalExp3} is a correct implementation of the Exp3 algorithm
  and has per-round running time of $O(\log N)$, where $N$ is the number of
  arms.
  %
\end{lemma}
\begin{proof}
  %
  The number of leaves in the modified interval tree never exceeds $N$, since
  every update we make to the weights is applied to one of the $N$ intervals of
  the form $[(i-1)/N, i/N)$ for $i \in [N]$. Therefore the sampling,
  integrating, and updating steps all cost $O(\log N)$ time per round.

  The algorithm maintains the following invariant: at every time $t$, suppose
  that $w_t$ is the weight function encoded by the modified interval tree. We
  are guaranteed that for all $\rho \in [(i-1)/N, i/N)$, $w_t(\rho_i)$ is equal
  to the weight that the Exp3 algorithm would store for arm $i$. Moreover, since
  each the intervals $[(i-1)/N, i/N)$ all have the same width, the probability
  that we sample a point belonging to the $i^{\rm th}$ interval is proportional
  to the constant weight on that interval. It follows that on each round, the
  algorithm samples an arm from the same distribution the Exp3 algorithm would.
  %
\end{proof}

\begin{algorithm}
\noindent \textbf{Parameter:} Step size $\lambda \in [0,1]$, number of arms $N$.
\begin{enumerate}[nosep, leftmargin=*]
\item Initialize $W$ to be the interval tree representing $w(\rho) = \ind{\rho \in [0,1]}$.
\item For $t = 1, \dots, T$
  \begin{enumerate}[nosep, leftmargin=*]
  \item Let $\rho_t \leftarrow \textsc{Draw}(W)$.
  \item Let $i_t = \lceil \rho_t / N \rceil$ be the index of the bin containing $\rho_t$.
  \item Play arm $i_t$ and observe it's loss $\ell_t(i_t)$.
  \item Let $\hat \ell_t \leftarrow \frac{\ell_t(\rho_t)}{p_t(A_t)}$, where $A_t = [(i-1)/N, i/N) \subset [0,1]$ and $p_t(A_t) \leftarrow \frac{\textsc{Integrate}(W, A_t)}{\textsc{Integrate}(W, [0,1])}$.
  \item Call $\textsc{Update}(W, A_t, \hat \ell_t)$.
  \end{enumerate}
\end{enumerate}
\caption{Efficient Implementation of Exp3}
\label{alg:IntervalExp3}
\end{algorithm}

